A Markov Random Field Topic Space Model for Document Retrieval

This paper proposes a novel statistical approach to intelligent document retrieval. It seeks to offer a more structured and extensible mathematical approach to the term generalization done in the popular Latent Semantic Analysis (LSA) approach to document indexing. A Markov Random Field (MRF) is presented that captures relationships between terms and documents as probabilistic dependence assumptions between random variables. From there, it uses the MRF-Gibbs equivalence to derive joint probabilities as well as local probabilities for document variables. A parameter learning method is proposed that utilizes rank reduction with singular value decomposition in a matter similar to LSA to reduce dimensionality of document-term relationships to that of a latent topic space. Experimental results confirm the ability of this approach to effectively and efficiently retrieve documents from substantial data sets.

==> lndscp.tex <==
\input rotate
\def\landscape#1{\setbox0=\vbox{
         \begin{minipage}{\textheight}#1\end{minipage}}
         \vbox to \textheight{\vfill\rotl{0}}}

\newcommand{\spt}{\mbox{$\; \; \; \; \; \; \; \; \; \; \; \; \;
\; \; \; \; \; \; \; \;$}}
\newcommand{\spe}{\mbox{$\; \; \; \; \; \; \; \; \; \; \;$}}
\newcommand{\spn}{\mbox{$\; \; \; \; \; \; \; \; \;$}}
\newcommand{\bve}{\mbox{\boldmath $ \varepsilon $}}
\newcommand{\bro}{\mbox{\boldmath $ \rho \! \! $ }}
\newcommand{\bfr}{\mbox{\bf $ r$}}

\newcommand{\al}{\mbox{$a_{L}$}}
\newcommand{\bal}{\mbox{\boldmath $a_{L}$}}
\newcommand{\as}{\mbox{$a_{S}$}}
\newcommand{\bas}{\mbox{\boldmath $a_{S}$}}
\newcommand{\dt}{\mbox{$\delta$}}
\newcommand{\bdt}{\mbox{\boldmath $\delta$}}
\newcommand{\fl}{\mbox{$F_{L}$}}
\newcommand{\bfl}{\mbox{\boldmath $F_{L}$}}
\newcommand{\fs}{\mbox{$F_{S}$}}
\newcommand{\bfs}{\mbox{\boldmath $F_{S}$}}

